Neural combinatorial optimization beyond the TSP: Existing architectures under-represent graph structure

Recent years have witnessed the promise that reinforcement learning, coupled with Graph Neural Network (GNN) architectures, could learn to solve hard combinatorial optimization problems: given raw input data and an evaluator to guide the process, the idea is to automatically learn a policy able to return feasible and high-quality outputs. Recent work have shown promising results but the latter were mainly evaluated on the travelling salesman problem (TSP) and similar abstract variants such as Split Delivery Vehicle Routing Problem (SDVRP). In this paper, we analyze how and whether recent neural architectures can be applied to graph problems of practical importance. We thus set out to systematically "transfer" these architectures to the Power and Channel Allocation Problem (PCAP), which has practical relevance for, e.g., radio resource allocation in wireless networks. Our experimental results suggest that existing architectures (i) are still incapable of capturing graph structural features and (ii) are not suitable for problems where the actions on the graph change the graph attributes. On a positive note, we show that augmenting the structural representation of problems with Distance Encoding is a promising step towards the still-ambitious goal of learning multi-purpose autonomous solvers.

==> workshop_instructions.tex <==
https://sites.google.com/view/gclr2022/submissions

We invite submissions to the AAAI workshop on Learning and Reasoning with Complex Graphs to be held virtually from February 22 - March 1, 2022 (the final date will be announced). We welcome the submissions in the following two formats:

Full papers: Submissions must represent original material that has not appeared elsewhere for publication and that is not under review for another refereed publication. Submissions may consist of up to 7 pages of technical content plus up to two additional pages solely for references.

Poster/Short/Position Papers: We encourage participants to submit preliminary but interesting ideas that have not been published before as short papers. These submissions would benefit from additional exposure and discussion that can shape a better future publication. We also invite papers that have been published at other venues to spark discussions and foster new collaborations. Submissions may consist of up to 4 pages plus one additional page solely for references.

The submissions should adhere to the AAAI paper guidelines available at (https://aaai.org/Conferences/AAAI-22/aaai22call/)

Accepted submissions will have the option of being published on the workshop website. For authors who do not wish their papers to be posted online, please mention this in the workshop submission. The submissions need not be anonymized.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Title: Should contain *Graph* *Neural/ML* *Edge features/node to edge/coordinates*
- From TSP to applied graph solutions: Can current Neural Graph xxx transfer?  
- Can Neural combinatorial optimization transfer to practical graph problems? 
- Existing do not take into account edge features

Results:
- It does not transfer
- Distance encoding helps
- Current architectures prefer coordinates

1) Introduction
2) Related
3) Transferring the problem:
Q: Qualitative assessment of how to transfer from TSP to other problems. Differences & similarities:
Node vs edge features, static versus dynamic
    3.1) Use cases:
        3.1.1) TSP/Split delivery/VRP
        3.1.2) Power/Channel
    3.2) Schematic view of existing architectures for the TSP
    3.3) Differences between the problems

% \textit{4) Experimental results 
% 4.1) Transferability : Transfer as is
% 4.2) Distance encoding to the rescue
4) "Transferability" results
\textit{Takeway}: GAT~GNN => Hypothesis: Edge features are not taken into account


Possibility 1:
5) Inability to take edge features into account
To verify the hypothesis, we test on the TSP without coordinates. We find bad results.
6) Distance encoding to the rescue
    5.1) "in theory" 
    5.2) DE on the power problem + 5.3) DE on TSP 

Possibility 2:
5) Distance encoding to the rescue
5.1) "in theory" 
5.2) DE on the power problem
5.3) back to the TSP for confirmation

5) Discussion and conclusions

New reference to add:
https://arxiv.org/pdf/2102.09544.pdf





